Prolonging the Hide-and-Seek Game: Optimal Trajectory Privacy for Location-Based Services

Human mobility is highly predictable. Individuals tend to only visit a few locations with high frequency, and to move among them in a certain sequence reflecting their habits and daily routine. This predictability has to be taken into account in the design of location privacy preserving mechanisms (LPPMs) in order to effectively protect users when they continuously expose their position to location-based services (LBSs). In this paper, we describe a method for creating LPPMs that are customized for a user's mobility profile taking into account privacy and quality of service requirements. By construction, our LPPMs take into account the sequential correlation across the user's exposed locations, providing the maximum possible trajectory privacy, i.e., privacy for the user's present location, as well as past and expected future locations. Moreover, our LPPMs are optimal against a strategic adversary, i.e., an attacker that implements the strongest inference attack knowing both the LPPM operation and the user's mobility profile. The optimality of the LPPMs in the context of trajectory privacy is a novel contribution, and it is achieved by formulating the LPPM design problem as a Bayesian Stackelberg game between the user and the adversary. An additional benefit of our formal approach is that the design parameters of the LPPM are chosen by the optimization algorithm.

==> evalintro.tex <==





\subsection{Computations Needed for Protecting Past and Present}\label{subsec:eval-pastpresent}

To compute the optimal LPPM described in Section~\ref{subsec:pastpresent}, we will take, for simplicity, $k=1$, i.e. there is only a single prior observation that matters $o_\text{pre} = o_\tau = o_{t-1}$, and the objective is to protect only the current and the previous locations, i.e. $a_\text{trg} = (r_t, r_\tau) = (r_t, r_{t-1})$. To determine $f$, we need to solve the associated linear program with objective \eqref{eq:pastpresentprivacy} and constraint \eqref{eq:pastpresentquality}. But, before we can solve the linear program, we need to specify values for $\psi(r_t, r_\tau | o_\tau) = \psi(r_t, r_{t-1} | o_{t-1})$. In the Appendix, we describe how this computation is performed in a recursive manner, depending on the actual value of $t$.

